Towards Better Long-range Time Series Forecasting using Generative Adversarial Networks

Long-range time series forecasting is usually based on one of two existing forecasting strategies: Direct Forecasting and Iterative Forecasting, where the former provides low bias, high variance forecasts and the later leads to low variance, high bias forecasts. In this paper, we propose a new forecasting strategy called Generative Forecasting (GenF), which generates synthetic data for the next few time steps and then makes long-range forecasts based on generated and observed data. We theoretically prove that GenF is able to better balance the forecasting variance and bias, leading to a much smaller forecasting error. We implement GenF via three components: (i) a novel conditional Wasserstein Generative Adversarial Network (GAN) based generator for synthetic time series data generation, called CWGAN-TS. (ii) a transformer based predictor, which makes long-range predictions using both generated and observed data. (iii) an information theoretic clustering algorithm to improve the training of both the CWGAN-TS and the transformer based predictor. The experimental results on five public datasets demonstrate that GenF significantly outperforms a diverse range of state-of-the-art benchmarks and classical approaches. Specifically, we find a 5% - 11% improvement in predictive performance (mean absolute error) while having a 15% - 50% reduction in parameters compared to the benchmarks. Lastly, we conduct an ablation study to demonstrate the effectiveness of the components comprising GenF.

==> table.tex <==
step    modify	ARIMA         True_Value	  cWGAN_GEP	    GPR		    SVR		    LSTM   cWGAN_GEP_w/o_MI                         cWGAN_GP               GAN
1       0.35	     nan		  75		    nan		    nan		    nan		    nan		nan		                                nan                    nan
2       0.7	         nan		  84		    nan		    nan		    nan		    nan		nan                                     nan                    nan
3       1.05	     nan		  78		    nan		    nan		    nan		    nan		nan                                     nan                    nan
4       1.4	         nan		  81		    nan		    nan		    nan		    nan		nan                                     nan                    nan
5       1.75	     nan		  64		    nan		    nan		    nan		    nan		nan                                     nan                    nan
6       2.1	         nan		  69		    nan		    nan		    nan		    nan		nan                                     nan                    nan
7       2.45	     nan		  66		    nan		    nan		    nan		    nan		nan                                     nan                    nan
8       2.8	         nan		  74		    nan		    nan		    nan		    nan		nan                                     nan                    nan
9       3.15	     nan		  66		    nan		    nan		    nan		    nan		nan                                     nan                    nan
10      3.5	         nan		  59		    nan		    nan		    nan		    nan		nan                                     nan                    nan
11      3.85	     nan		  72		    nan		    nan		    nan		    nan		nan                                     nan                    nan
12      4.2	         nan		  80		    nan		    nan		    nan		    nan		nan                                     nan                    nan
13      4.55         nan		  82		    nan		    nan		    nan		    nan		nan                                     nan                    nan
14      4.9	         nan		  85		    nan		    nan		    nan		    nan		nan                                     nan                    nan
15      5.25         nan		  89		    nan		    nan		    nan		    nan		nan                                     nan                    nan
16      5.6	         nan		  79		    nan		    nan		    nan		    nan		nan                                     nan                    nan
17      5.95         nan		  80		    nan		    nan		    nan		    nan		nan                                     nan                    nan
18      6.3	         nan		  77		    nan		    nan		    nan		    nan		nan                                     nan                    nan
19      6.65         nan		  83		    nan		    nan		    nan		    nan		nan                                     nan                    nan
20      7	          77		  77		    77		    77		    77		    77		77                                      77                      77
21      9.625  76.8648799		  68		    71.458		71.85		74.01		72.2	72.9			                        74.4                   75.1
22      12.25  80.17638956		  70		    72.976		67.87		75.43		75.5	74.9                                    76.1                   75.7
23      14.87  77.58801317		  71		    71.797		76.6		77.43		74.5	74.2                                    75.5                   76.2
24      17.5   84.55		      77		    78.97		76.8		79.66		78.1	79.24                                   80.34                  80.72
25      20.12  77.65		      74		    76.66		80.6		79.88		74.7	76.88                                   79.23                  79.58
26      22.75  78.40	          81		    83.23		78.7		76.24		78.2	84.72                                   83.79                  85.15
27      25.37  77.95	          83		    81.25		79.94		78.48		78.3	81.58                                   78.02                  78.53
28      28	   69.20	          75		    72.26		69.32		69.52		70.25	78.87                                   78.02                  79.57


==> table_109.tex <==
step    modify	     ARIMA         True_Value	  cWGAN_GEP	    GPR		    SVR		   LSTM	 cWGAN_GEP_w/o_MI                         cWGAN_GP                GAN
1       0.35	     nan		        98		    nan		    nan		    nan		    nan		nan		                                nan                    nan
2       0.7	         nan		        94		    nan		    nan		    nan		    nan		nan                                     nan                    nan
3       1.05	     nan		        97		    nan		    nan		    nan		    nan		nan                                     nan                    nan
4       1.4	         nan		        98		    nan		    nan		    nan		    nan		nan                                     nan                    nan
5       1.75	     nan		        95		    nan		    nan		    nan		    nan		nan                                     nan                    nan
6       2.1	         nan		        84		    nan		    nan		    nan		    nan		nan                                     nan                    nan
7       2.45	     nan		        91		    nan		    nan		    nan		    nan		nan                                     nan                    nan
8       2.8	         nan		        103		    nan		    nan		    nan		    nan		nan                                     nan                    nan
9       3.15	     nan		        95		    nan		    nan		    nan		    nan		nan                                     nan                    nan
10      3.5	         nan		        91		    nan		    nan		    nan		    nan		nan                                     nan                    nan
11      3.85	     nan		        95		    nan		    nan		    nan		    nan		nan                                     nan                    nan
12      4.2	         nan		        92		    nan		    nan		    nan		    nan		nan                                     nan                    nan
13      4.55         nan		        97		    nan		    nan		    nan		    nan		nan                                     nan                    nan
14      4.9	         nan		        91		    nan		    nan		    nan		    nan		nan                                     nan                    nan
15      5.25         nan		        90		    nan		    nan		    nan		    nan		nan                                     nan                    nan
16      5.6	         nan		        84		    nan		    nan		    nan		    nan		nan                                     nan                    nan
17      5.95         nan		        95		    nan		    nan		    nan		    nan		nan                                     nan                    nan
18      6.3	         nan		        97		    nan		    nan		    nan		    nan		nan                                     nan                    nan
19      6.65         nan		        94		    nan		    nan		    nan		    nan		nan                                     nan                    nan
20      7	          92		        92		    92		    92		    92		    92		92                                       92                      92
21      9.625        86.8		        85		    85.3	    88.8		84.3	    83.5	85.6			                        86.7                   82.1
22      12.25        89.9	            89		    88.6	    87.1		92.9		90.7    87.8                                    91.3                   87.2
23      14.87        83.9		        86		    85.1		84.2		85.1		87.3    84.7                                    87.8                   87.8
24      17.5    	 89.55	            85		    87.09		87.8	    90.6		88.1	87.55                                   87.97                  83.41
25      20.12        87.68	            85		    86.33		82.1		85.98	    87.38	86.48                                   87.23                  87.58
26      22.75        81.40	            82		    84.41		80.7		88.24		86.21	85.49                                   85.88                  84.51
27      25.37        79.95	            82		    84.02		77.2	    81.48		85.43	85.03                                   84.97                  85.53
28      28	         85.20	            80		    82.95		83.2		83.42		83.25	83.79                                   84.83                  85.92


==> table_890.tex <==
step    modify	ARIMA         True_Value	  cWGAN_GEP	    GPR		    SVR		    LSTM   cWGAN_GEP_w/o_MI                cWGAN_GP                  GAN
1       0.35	 nan		        84		    nan		    nan		    nan		    nan		nan		                          nan                    nan
2       0.7	     nan		        70		    nan		    nan		    nan		    nan		nan                               nan                    nan
3       1.05	 nan		        66		    nan		    nan		    nan		    nan		nan                               nan                    nan
4       1.4	     nan		        69		    nan		    nan		    nan		    nan		nan                               nan                    nan
5       1.75	 nan		        67		    nan		    nan		    nan		    nan		nan                               nan                    nan
6       2.1	     nan		        75		    nan		    nan		    nan		    nan		nan                               nan                    nan
7       2.45	 nan		        83		    nan		    nan		    nan		    nan		nan                               nan                    nan
8       2.8	     nan		        82		    nan		    nan		    nan		    nan		nan                               nan                    nan
9       3.15	 nan		        91		    nan		    nan		    nan		    nan		nan                               nan                    nan
10      3.5	     nan		        90		    nan		    nan		    nan		    nan		nan                               nan                    nan
11      3.85	 nan		        83		    nan		    nan		    nan		    nan		nan                               nan                    nan
12      4.2	     nan		        82		    nan		    nan		    nan		    nan		nan                               nan                    nan
13      4.55     nan		        91		    nan		    nan		    nan		    nan		nan                               nan                    nan
14      4.9	     nan		        90		    nan		    nan		    nan		    nan		nan                               nan                    nan
15      5.25     nan		        83		    nan		    nan		    nan		    nan		nan                               nan                    nan
16      5.6	     nan		        82		    nan		    nan		    nan		    nan		nan                               nan                    nan
17      5.95     nan		        83		    nan		    nan		    nan		    nan		nan                               nan                    nan
18      6.3	     nan		        84		    nan		    nan		    nan		    nan		nan                               nan                    nan
19      6.65     nan		        80		    nan		    nan		    nan		    nan		nan                               nan                    nan
20      7	     80		            80		    80		     80		    80		    80		80                                80                     80
21      9.625  	 87.3			    84		    82.1	    88.1		79.8	    86.8    81.7			                  81.2                   80.7
22      12.25 	 67.2			    73		    75.3		77.3		77.5		70.4	75.7                              77.1                   78.3
23      14.87  	 79.3			    76		    78.2		72.2	    73.1		79.8	78.6                              72.6                   73.2
24      17.5     77.71			    75		    75.58		78.51		76.96		76.83	76.21                             76.59                  77.03
25      20.12  	 72.33			    67		    71.23		71.25	    70.58		72.58   71.98                             74.28                  73.99
26      22.75    63.04			    66		    67.77		70.87		71.41		68.44	68.07                             68.29                  68.48
27      25.37  	 65.58			    71		    71.98		66.95		75.48		73.27	72.29                             70.23                  73.09
28      28	     74.20			    72		    74.58		74.23		74.92		75.51   75.02                             75.47                  75.88

